Hearing the voice of experts: Unveiling Stack Exchange communities' knowledge of test smells

Refactorings are transformations to improve the code design without changing overall functionality and observable behavior. During the refactoring process of smelly test code, practitioners may struggle to identify refactoring candidates and define and apply corrective strategies. This paper reports on an empirical study aimed at understanding how test smells and test refactorings are discussed on the Stack Exchange network. Developers commonly count on Stack Exchange to pick the brains of the wise, i.e., to `look up' how others are completing similar tasks. Therefore, in light of data from the Stack Exchange discussion topics, we could examine how developers understand and perceive test smells, the corrective actions they take to handle them, and the challenges they face when refactoring test code aiming to fix test smells. We observed that developers are interested in others' perceptions and hands-on experience handling test code issues. Besides, there is a clear indication that developers often ask whether test smells or anti-patterns are either good or bad testing practices than code-based refactoring recommendations.

==> Chapters/Background.tex <==
\section{Background}\label{sec:Background}

In this section, we present some key concepts needed to deepen the discussion about smells in test code, refactoring, and software development forum.

\subsection{Test smells}

According to Beck et al. \cite{beck2003test}, %it is important to have well-designed test code that respects good design principles because it makes test cases easier to comprehend, and maintain and can be successfully exploited to diagnose problems in production code.
it is important that tests are coded following good design principles, so that the test is well designed and therefore easier to maintain. Tests explored without difficulties are able to diagnose problems in production code effectively.

Inspired by these arguments, van Deursen et al. \cite{Deursen2001_TestRefactoring} report that poorly designed test cases describe symptoms that can indicate possible design problems in the test code. These problems are called Test Smells. Test smells are anti-patterns in unit test code that developers have implemented \cite{Garousi2018_SurveySmells,Peruma2019_DistributionAndroid, Spadini2020_SeverityThresholds}.\looseness=-1 %and differ from those defined by Fowler et al. \cite{fowler2018refactoring} for production code and are based on how the test cases are organized, implemented, and interact with each other. %van Deursen et al. \cite{van2001refactoring} defined the first catalog of 11 anti-patterns in unit test code. Besides van Deursen et al. \cite{van2001refactoring}, other catalogs were extended \cite{Meszaros2003_AutomationManifesto, Garousi2018_SurveySmells}.

The presence of test smells in test code can be interpreted as an indicator of poor software quality, resulting in a miscomprehensive and difficult to maintain test code \cite{greiler2013automated}. % In this study, we analyzed of test smells Assertion Roulette (AR), Eager Test (ET), Empty Test (EpT), Lazy test (LT), Redundant Assertion (RA), Unknown Test (UT), Sensitive Equality (SE), General Fixture (GF), Resource Optimism (RO), Exception Catch/Throw (ECT), Print Statement (PS), Sleepy Test (ST), Duplicate Assert (DA), Ignored Test (IgT), Magic Number Test (MNT), Verbose Test (VT), Conditional Test Logic (CTL), Mystery Guest (MG).

\subsection{Refactoring}

Refactoring is a change that reorganizes software code without changing its functionality \cite{fowler2018refactoring}. For production and test codes, behavior has multiple meanings. The behavior of production code refers to the effects of its execution, such as return values, variable changes, and impacts on external resources. The test code checks whether the behavior of the refactored code has not changed after refactoring the production code \cite{Deursen2001_TestRefactoring, fowler2018refactoring}. On the other hand, the production code verification is referred to by the test code behavior. A verification consists of one assertion and actions to check the production code. When test code is refactored, the test suite's results before and after the refactoring must be the same \cite{Guerra2007_Refactoring_Safely}.


%\textbf{Code Review.}

\subsection{Collaborative discussion forums}

The competence of software engineering practitioners is tied to a lifelong quest for knowledge, and educational circles are excellent environments for spreading knowledge\cite{StackExchange}. According to \cite{Tahir2020_CodeSmells}, practitioners often gather in online forums and similar portals in search of critical discourse on software development issues, including anti-patterns. For example, \textit{Stack Exchange} is a website network of collaborative discussion forums (\textit{Stack Overflow}, \textit{Software Engineering}, and \textit{Code Review}) that offers insightful resources on development issues, besides as educating developers on best practices \cite{Tahir2020_CodeSmells}. As mentioned in \cite{StackExchange}, participating in and sustaining learning communities is a durable and valuable aspect of professional life.

\textit{Stack Overflow} is the most popular Questions and Answers (Q\&A) forum for software development \cite{Openja2020_ReleaseEngineering, bhasin2021student}. Stack Overflow was founded in 2008 and has over 21 million Questions asked to date. \textit{Stack Overflow} questions involve technical and general discussions on various topics, covering questions related to software engineering. On the other hand, the \textit{Software Engineering} forum consists of a more centralized environment for discussions about the software development life cycle \cite{Tahir2020_CodeSmells}.

Figure  \ref{fig:post-example}  is an example of a post extracted from StackOverflow\footnote{Available at \hyperlink{https://stackoverflow.com/questions/10781050}{https://stackoverflow.com/questions/10781050}}, where the author asks if the practice adopted by him in the \texttt{JUnit} test case consists of duplication and how his test can be written without duplication. Figure \ref{fig:answer-example} shows a user's response referring to the post of Figure \ref{fig:post-example}. The answer informs that the practice adopted by the author of the post is a test anti-pattern called the ugly mirror. As a possible solution, the respondent suggested simplifying the test code, i.e., avoiding conditional structures and using only assertions. Also, it was suggested to create a test object to run the tests manually for complex data structures. The post's author rated the answer as accepted, and the answer got four votes.

\begin{figure}[htbp]
{\includegraphics[width=1.0\linewidth]{images/post-example.png}}
\caption{Example post}
\label{fig:post-example}
\end{figure}

\begin{figure}[htbp]
{\includegraphics[width=1.0\linewidth]{images/answer-example.png}}
\caption{Example answer}
\label{fig:answer-example}
\end{figure}
